Key-Point-Driven Data Synthesis with its Enhancement on Mathematical Reasoning

Large language models (LLMs) have shown great potential in complex reasoning tasks, yet their performance is often hampered by the scarcity of high-quality and reasoning-focused training datasets. Addressing this challenge, we propose Key-Point-Driven Data Synthesis (KPDDS), a novel data synthesis framework that synthesizes question-answer pairs by leveraging key points and exemplar practices from authentic data sources. KPDDS ensures the generation of novel questions with rigorous quality control and substantial scalability. As a result, we present KPMath, an extensive synthetic dataset tailored for mathematical reasoning, comprising over 800K question-answer pairs. Utilizing KPMath and augmenting it with additional reasoning-intensive corpora, we create the comprehensive KPMath-Plus dataset. The Qwen1.5-72B model, fine-tuned on KPMath-Plus, achieves 87.0% PASS@1 accuracy on GSM8K and 58.3% on MATH, surpassing competitors in the 7B to 70B range and best commercial models like GPT-4 across multiple math reasoning datasets.

==> figs/ablation.tex <==
% \begin{figure}[t]
%     \begin{minipage}{0.48\textwidth}
%         \centering
%         \includegraphics[width=1.0\textwidth]{figs/new_figs/voting.pdf}
%         \caption{Training Results with Different Voting Strategies (average performance on six mathematical dataset).}
%         \label{fig:ab_threshold}
%     \end{minipage}
%     \label{fig:figures}
% \end{figure}

% \begin{wrapfigure}{R}{0.5\textwidth}
%     \vskip -0.15in
%     \includegraphics[width=\linewidth]{figs/new_figs/voting.pdf}
%     \vskip -0.1in
% \caption{Training Results with Different Voting Strategies (average performance on six mathematical dataset).}
% \label{fig:ab_threshold}
% \end{wrapfigure}

% \begin{figure}[t]
%     \centering
%     \begin{subfigure}{0.43\textwidth}
%         \centering
%     \includegraphics[width=1.0\textwidth]{figs/dataset.pdf}
%         \caption{}
%         \label{fig:dataset}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.54\textwidth}
%         \centering
%     \includegraphics[width=1.0\textwidth]{figs/threshold.pdf}
%         \caption{}
%         \label{fig:ab_threshold}
%     \end{subfigure}
%     \caption{(a) Comparative analysis of fine-tuning results on Mistral-7B using various datasets, illustrating both the total number and the synthetic number of data samples. (b) Comparative analysis of the minimum acceptable score in the CSV.}
%     \label{fig:figures}
% \end{figure}


==> figs/error_q_case.tex <==
% \setlength{\columnsep}{0.1cm}
\begin{figure}[t]

\begin{minipage}{1\textwidth}
\begin{tcolorbox}[colback=msyellow!5!white,colframe=msyellow!80!black, fontupper=\small]
\textbf{Question}:
You are designing a rectangular garden where the length is expressed as $x$ feet. The length of the garden can be decomposed into its integer and fractional parts such that $\lfloor x \rfloor + x = \frac{25}{2}$. The width of the garden is 7 feet less than its length. Find the ratio of the width of the garden to its perimeter. Express your answer in the form $a:b$.
\Sepline
\textbf{Solution}: First, we need to find the length of the garden. We can write $x$ as $n+\dfrac{1}{2}$, where $n$ is the greatest integer less than $x.$ Therefore, we can write $\lfloor x \rfloor + x$ as $n+n+\dfrac{1}{2}=\dfrac{25}{2}$. Solving, we get $n=6$. Therefore, the length of the garden is $6+\dfrac{1}{2}=6.5$ feet.
Next, we calculate the width of the garden, which is 7 feet less than its length. Therefore, the width is $6.5 - 7 = -0.5$ feet. This is not possible, as the width cannot be negative. Therefore, there must be an error in the question. The answer is: Error in the question
\end{tcolorbox}
\end{minipage}

\caption{An example of wrong question in KPMath.}
\label{fig:wrong_q_example}
\end{figure}


==> figs/labeling_example.tex <==
\setlength{\columnsep}{0.2cm}
\begin{figure}[t]
\begin{tcolorbox}[colback=msblue!5!white,colframe=msblue!80!black, fontupper=\small]
\textbf{Prompt for KPs Generation:}\\ 
As a mathematics education specialist, please analyze the topics and knowledge points of the provided question and its answer. These analysis should serve as a guide for teachers to craft analogous problems and as focal learning objectives for students when approaching the problem. Be sure to avoid repetition of Knowledge Points for clarity and conciseness. Specific requirements are as follows: 

1. Identify and categorize the main mathematical topics involved in the problem.  If knowledge from non-mathematical fields is used, it is classified into Others - xxx, such as Others - Problem Context.

2. For each topic, enumerate the essential Knowledge Points relevant to the problem. 
\end{tcolorbox}
\begin{tcolorbox}[colback=msgreen!5!white,colframe=msgreen!80!black, fontupper=\small]
\textbf{Seed Problem:}\\ 
The points $(9, -5)$ and $(-3, -1)$ are the endpoints of a diameter of a circle. What is the sum of the coordinates of the center of the circle?

The center of the circle is located at the midpoint of any diameter. Thus, the center of the circle is $\left(\frac{9+(-3)}{2}, \frac{(-5)+(-1)}{2}\right) = (3, -3)$. The sum of the coordinates of the center of the circle is therefore $3 + (-3) = \boxed{0}$.
\Sepline
\textbf{Knowledge Points:}\\ 
Geometry - Circles: 
\vspace{-0.2em}
\begin{itemize}[leftmargin=0.5cm, rightmargin=0.2cm]
    \setlength{\itemsep}{-0.2em}
    % \setlength{\itemindent}{-0.2em}
    \item Understanding that the center of a circle is the midpoint of its diameter
    \item Application of the midpoint formula to find the center of a circle given the endpoints of a diameter
\end{itemize}
\vspace{-0.2em}
Algebra - Coordinate Geometry: 
\vspace{-0.2em}
\begin{itemize}[leftmargin=0.5cm, rightmargin=0.2cm]
    \setlength{\itemsep}{-0.2em}
    \item Understanding of coordinate points and how to manipulate them
    \item Ability to add and subtract coordinates
\end{itemize}
% \{
% "Geometry - Circles": ["Understanding that the center of a circle is the midpoint of its diameter", "Application of the midpoint formula to find the center of a circle given the endpoints of a diameter"],

% "Algebra - Coordinate Geometry": ["Understanding of coordinate points and how to manipulate them", "Ability to add and subtract coordinates"]
% \}
\end{tcolorbox}
% \vspace{-1em}
\caption{The prompt to label mathematical topics and KPs and an example of the mathematical KPs generated by GPT-4. We use few-shot prompt in experiment to ensure the output format.}
\label{fig:label_example}
\end{figure}

==> figs/prompt_eval_q.tex <==
% \setlength{\columnsep}{0.2cm}
\begin{figure}[ht]
\begin{tcolorbox}[colback=msblue!5!white,colframe=msblue!80!black,fontupper=\small]
\textbf{Prompt for Question Evaluation}\\ 
You are a math professor. Would you please evaluate the answer for the problem for me? 
Tips:

* Verify that the mathematical concepts and theorems used are correct and applicable to the context of the problem.

* Check if the statement of the problem is clear and unambiguous, and that it aligns with the assumptions made during the solution process.

* Step through the solution process, resolve each mathematical calculation again, and then compare with the original answer for accuracy.

* Ensure that the solution steps are logically coherent, with no omissions or unreasonable inferences.

* Confirm that the final result of the solution addresses the requirements of the problem and is consistent with the way the question is posed.

The evaluation score should be a float number between 0 and 1. The higher the number is, the better the answer is.
\end{tcolorbox}
% \vspace{-1em}
\caption{?}
\label{fig:prompts}
\end{figure}


==> figs/prompt_kps.tex <==
\setlength{\columnsep}{0.2cm}
\begin{figure}[h]
\begin{minipage}[b]{0.48\textwidth}
\begin{algorithm}[H]
\small
    \caption{CPM Calculation}
    \label{alg:co_occurrence}
    \begin{algorithmic}[1]
    \REQUIRE MPKPP $data$
    \STATE $N \gets$  number of topics in $data$
    \STATE Initialize $CPM$ with zeros of shape $N \times N$
    \FOR{each $d$ in $data$}
        \FOR{each topic $i$ in $d$}
            \FOR{each topic $j$ in $d$}
                \IF{$i \neq j$}
                    \STATE $CPM[i][j] += 1$
                \ENDIF
            \ENDFOR
            \IF{Number of KPs in topic $i > 5$}
                \STATE $CPM[i][i] += 1$
            \ENDIF
        \ENDFOR
    \ENDFOR
    \STATE $CPM \gets \log_{10}(CPM + 1)$
    \RETURN $CPM$
    \end{algorithmic}
\end{algorithm}
\end{minipage}%
\begin{minipage}[b]{0.48\textwidth}
\begin{tcolorbox}[colback=msblue!5!white,colframe=msblue!80!black, fontupper=\small] 
%height = 0.4\textwidth]
\textbf{Prompt for KPs Generation:}\\ 
As a mathematics education specialist, please analyze the topics and knowledge points of the provided question and its answer. These analysis should serve as a guide for teachers to craft analogous problems and as focal learning objectives for students when approaching the problem. Be sure to avoid repetition of Knowledge Points for clarity and conciseness. Specific requirements are as follows: 

1. Identify and categorize the main mathematical topics involved in the problem.  If knowledge from non-mathematical fields is used, it is classified into Others - xxx, such as Others - Problem Context.

2. For each topic, enumerate the essential Knowledge Points relevant to the problem. 
\end{tcolorbox}
\caption{The prompt to label mathematical topics and KPs.}
\label{fig:label_example}
\end{minipage}
\end{figure}


==> sections/0-Intruduction.tex <==
\section{Introduction}

Nowadays, large language models (LLMs) like GPT-4 \citep{openai2023gpt4}, Gemini \citep{team2023gemini}, and Mistral \citep{mistral2024large} have displayed impressive capabilities that are being harnessed in various fields \cite{bubeck2023sparks}, attracting lots of interests in the community of artificial intelligence.
However, there are debates on the reasoning ability of LLMs and some works question the reasoning abilities of LLMs in tasks that require strong reasoning skills like difficult math word problems \citep{lewkowycz2022solving}, competition-level programming problems \citep{huang2023competition} and planning with both vision and language \citep{cen2024using}.

It can be understood from the low data output ratio during the collection process of the current math reasoning corpus like OpenWebMath \citep{paster2023openwebmath} and MathPile \citep{wang2023generative} and the analysis of math reasoning benchmark, like the MATH dataset \citep{hendrycksmath2021}, that the scarcity of reasoning-related data in the overall training data and the absence of clear reasoning steps, such as detailed math problem solutions or complex task strategies, are two factors that limit the performance of current LLMs on complex reasoning tasks.

Previous studies like ToRA \citep{gou2023tora}, MetaMath \citep{yu2023metamath} and MMIQC \citep{liu2024augmenting} have demonstrated that more data can be obtained by either rephrasing questions, exposing the reasoning process of existing question-answer pairs either in chain-of-thought (CoT) style \citep{wei2022chain} or program-based \citep{yue2023mammoth, gou2023tora} style, or generating new questions.
\cref{fig:dataset} illustrates the zero-shot PASS@1 accuracies of some models on MATH dataset.
These models are Mistral-7B \citep{jiang2023mistral} finetuned on different synthetic datasets with different scales and generate with CoT-style answers in inference.
We can see that with more total amount of SFT data, the performance will be better.
Therefore, we believe that existing foundation models can improve their reasoning abilities by learning from large-scale input-output pairs with explicit reasoning steps directly without modifying model architectures.

\input{figs/main_figure}

In this work, we focus on how to synthesize high-quality training data based on existing symbolic knowledge and datasets and use such data to improve the foundation model’s reasoning skills.
According to our study, there are three key aspects for data synthesis in math reasoning: \textbf{question novelty}, \textbf{quality control} and \textbf{data scalability}, and it is difficult to do well in all these aspects.
We consider all these aspects and propose a new synthetic question-answer pair dataset \textbf{KPMath} for math reasoning, whose pipeline is depicted in \cref{fig:flow_chart}.
(1) First, we start from the problems in the training set of the MATH dataset as the seed, employing a labeling model to extract the topics and key points.
After applying a clustering algorithm for deduplication and alignment, we get 119 topics and 23,827 key points as the knowledge in math.
(2) Second, a synthesizing model is applied to generate new questions controlled by merging key points of two or more mathematical topics, and a scoring model is used to estimate the qualities of generated questions before the next step.
Please note that for each topic, we provide an example question-answer pair as the explanation.
Since the target of synthetic data is to provide a fuller and more realistic representation of the original data source, we also estimate a co-occurrence probability matrix for better sampling the topics.
(3) Third, we construct several answers for each generated question that pass the quality assessment by prompting a reasoning model and merge them to consensus solutions by voting.
(4) At last, the generated questions are expanded by a rephrasing model and combined with the consensus solutions to form the KPMath dataset.

As far as we know, KPMath is the largest synthetic question-answer pair dataset for math reasoning, consisting 1.01M question-answer pairs.
Following \cite{liu2024augmenting}, we further combine MMIQC \citep{liu2024augmenting} and the CoT part of MathInstruct \citep{yue2023mammoth} with KPMath to formulate a comprehensive training dataset \textbf{KPMath-Plus}.
SFT experiments of Mistral-7B \citep{jiang2023mistral} on KPMath-Plus indicate that the finetuned model outperformances other 7B models without code usage, even surpassing some 34B models in terms of zero-shot PASS@1 accuracy on MATH test set.
Moreover, The data contamination test following \cite{azerbayev2023llemma} indicates a very low risk of data contamination for KPMath.

In summary, our contributions include the following:
\begin{itemize}
\item We propose a new pipeline for synthesizing data for math reasoning, which involves topics and key points inferred from real data and question-answer exemplar pairs as controlling factors. As far as we know, the synthetic dataset KPMath is the largest synthetic data for math reasoning.
\item Mistral-7B models finetuned on KPMath-Plus achieve a better zero-shot PASS@1 accuracy of 7B models in the MATH test set than compared baselines without code usage, even surpassing a group of 34B models.
\item We explore quality control for both question and answer. Our key points are inferred from existing real data, which not only leads to more diverse and novel questions but also can be enhanced with clearer explanations like question-answer exemplar pairs.
\end{itemize}


==> tables/ab_result1.tex <==
\begin{table*}[t]
\small
\centering
\setlength\tabcolsep{2pt}
\caption{Performance comparison of different data components across MATH subtopics (\%).}
\label{tab:ab_components}
% \vskip 0.15in
\resizebox{1.0\textwidth}{!}{
\begin{tabular}{lccccccccc}
\toprule
Dataset & \# Samples   &  \makecell{Intermediate\\Algebra} & \makecell{Counting \\\& Probability}  & Precalculus & Geometry & \makecell{Number\\Theory} & Algebra & Prealgebra &  Overall \\
\midrule
%KPMath & 1.01M \\
MMIQC           & 2.29M & 17.2 & 28.7 & 20.3 & 28.2 & 27.8 & 55.0 & 55.6 & 36.5\\
MMIQC + KPMath & 3.3M  & \underline{18.8} & \underline{34.6} & \textbf{23.4} & \underline{29.2} & \underline{29.3} & \textbf{57.7} & \underline{56.7} & \underline{38.8} \\
MMIQC + MI-CoT  & 2.85M & 18.2 & 31.4 & 22.5 & \underline{29.2} & 28.9 & 53.4 & 54.9 & 36.9 \\
MMIQC + MI-CoT + KPMath & 3.86M & \textbf{19.5} & \textbf{33.8} & \textbf{23.4} & \textbf{30.3} & \textbf{31.1} & \underline{56.9} & \textbf{58.9} & \textbf{39.3} \\
\bottomrule
\end{tabular}}
% \vskip -0.1in
\end{table*}



==> tables/ab_result2.tex <==
\begin{table*}[t]
\small
\centering
\setlength\tabcolsep{2pt}
\caption{Comparative analysis of model performance on MATH subtopics with and without erroneous questions (\%).}
\label{tab:wrong_q}
% \vskip 0.15in
\begin{center}
% \begin{small}
\resizebox{1.0\textwidth}{!}{
\begin{tabular}{lccccccccc}
\toprule
Dataset & \# Samples   &  \makecell{Intermediate\\Algebra} & \makecell{Counting \\\& Probability}  & Precalculus & Geometry & \makecell{Number\\Theory} & Algebra & Prealgebra &  Overall \\
\midrule
KPMath-Plus  & 3.86M & 19.5 & 33.8 & 23.4 & 30.3 & 31.1 & 56.9 & 58.9 & 39.3\\
\quad - ErrorQ  & 3.79M & 17.4 & 33.3 & 23.3 & 32.6 & 28.0 & 56.4 & 56.5 & 38.2\\
\bottomrule
\end{tabular}}
% \end{small}
\end{center}
% \vskip -0.1in
\end{table*}



==> tables/contamination.tex <==

\begin{lstlisting}[breaklines=true,, basicstyle=\small]

input:  257
A square is drawn such that one of its sides coincides with the line $y = 7$, and so that the endpoints of this side lie on the parabola $y = 2x^2 + 8x + 4$. What is the area of the square?
overlap: 
A square is drawn such that one of its sides coincides with the line $y = 7$, and so that the endpoints of this side lie on the parabola $y =
>>>>>>>>

input:  2314
Let $x,$ $y,$ and $z$ be nonnegative real numbers such that $x + y + z = 3.$ Find the maximum value of \[(xy + z)(xz + y).\]
overlap: 
$x,$ $y,$ and $z$ be nonnegative real numbers such that $x + y + z = 3.$ Find the maximum value of
>>>>>>>>

input:  2253
For some real numbers $a$ and $b$, the equation \[ 8x^3 + 4ax^2 + 2bx + a = 0 \]has three distinct positive roots. If the sum of the base-2 logarithms of the roots is 5, what is the value of $a$?
overlap: 
three distinct positive roots. If the sum of the base-2 logarithms of the roots is 5, what is the value of
>>>>>>>>

input:  4974
Find the matrix $\mathbf{M}$ that swaps the rows of a matrix. In other words, \[\mathbf{M} \begin{pmatrix} a & b \\ c & d \end{pmatrix} = \begin{pmatrix} c & d \\ a & b \end{pmatrix}.\]If no such matrix $\mathbf{M}$ exists, then enter the zero matrix.
overlap: 
\begin{pmatrix} a & b \\ c & d \end{pmatrix} = \begin{pmatrix} c & d \\ a & b \end{pmatrix}.\]If no such matrix
>>>>>>>>

input:  2416
Let $a,$ $b,$ $c,$ and $d$ be positive real numbers such that $a + b + c + d = 10.$ Find the maximum value of $ab^2 c^3 d^4.$
overlap: 
Let $a,$ $b,$ $c,$ and $d$ be positive real numbers such that $a + b + c + d =
>>>>>>>>

input:  1042
Suppose the function $f(x)$ is defined explicitly by the table $$\begin{array}{c || c | c | c | c | c} x & 0 & 1 & 2 & 3 & 4 \\ \hline f(x) & 0 & 0 & 1 & 3 & 6 \end{array}$$ This function is defined only for the values of $x$ listed in the table. Suppose $g(x)$ is defined as $f(x)-x$ for all numbers $x$ in the domain of $f.$ How many distinct numbers are in the range of $g(x)?$
overlap: 
$$\begin{array}{c || c | c | c | c | c} x & 0 & 1 & 2 & 3 & 4 \\ \hline
>>>>>>>>

input:  1972
In the diagram, the two triangles shown have parallel bases. What is the ratio of the area of the smaller triangle to the area of the larger triangle? Express your answer as a common fraction. [asy] path p = (0,0)--dir(-60)--dir(-120)--(0,0); draw(p); draw(scale(3)*p); label("4 cm",dir(-60)--dir(-120),S); label("10 cm",3*dir(-60)--3dir(-120),S); [/asy]
overlap: 
What is the ratio of the area of the smaller triangle to the area of the larger triangle? Express your answer as a common fraction. [asy]
>>>>>>>>

input:  1917
Points $A(0,0), B(9,6)$ and $C(6,12)$ are vertices of triangle $ABC$. Point $D$ is on segment $AB$ such that $2(AD) = DB$, point $E$ is on segment $BC$ such that $2(BE) = EC$ and point $F$ is on segment $CA$ such that $2(CF) = FA$. What is the ratio of the area of triangle $DEF$ to the area of triangle $ABC$? Express your answer as a common fraction.
overlap: 
= FA$. What is the ratio of the area of triangle $DEF$ to the area of triangle $ABC$? Express your answer as a common fraction.
>>>>>>>>

input:  3166
The greatest common divisor of two integers is $(x+3)$ and their least common multiple is $x(x+3)$, where $x$ is a positive integer. If one of the integers is 40, what is the smallest possible value of the other one?
overlap: 
integers is $(x+3)$ and their least common multiple is $x(x+3)$, where $x$ is a positive integer. If one of the integers is 40, what is the smallest possible value of
>>>>>>>>

output:  3232
Let us look at the powers of $5$: \begin{align*} 5^1 &\equiv 5 \pmod{7} \\ 5^2 &\equiv 4 \pmod{7} \\ 5^3 &\equiv 6 \pmod{7} \\ 5^4 &\equiv 2 \pmod{7} \\ 5^5 &\equiv 3 \pmod{7} \\ 5^6 &\equiv 1 \pmod{7}. \end{align*} Since $5^6 \equiv 1 \pmod{7},$ we see that $5^{30} \equiv (5^6)^5 \equiv 1 \pmod{7},$ hence our desired remainder is $\boxed{1}.$
overlap: 
\begin{align*} 5^1 &\equiv 5 \pmod{7} \\ 5^2 &\equiv 4 \pmod{7} \\ 5^3 &\equiv 6 \pmod{7} \\ 5^4 &\equiv 2 \pmod{7} \\ 5^5 &\equiv 3 \pmod{7} \\ 5^6 &\equiv 1 \pmod{7}.
>>>>>>>>

output:  1445
We can just treat the knot as another bead. There are $5!$ ways to place the beads and the knot on the bracelet, but we must divide by 5 for rotational symmetry (5 rotations for each arrangement), and by 2 for reflectional symmetry (we can flip the bracelet to get the same arrangement). The answer is $\dfrac{5!}{5 \times 2} = \boxed{12}$.
overlap: 
on the bracelet, but we must divide by 5 for rotational symmetry (5 rotations for each arrangement), and by 2 for reflectional symmetry (we can flip the bracelet to get the same arrangement). The answer is $\dfrac{5!}{5 \times 2} =
>>>>>>>>

output:  3528
The primes between 1 and 100 are 2, 3, 5, 7, 11, 13, 17, 19, 23, 29, 31, 37, 41, 43, 47, 53, 59, 61, 67, 71, 73, 79, 83, 89, and 97. We compute their residues modulo 16: 2, 3, 5, 7, 11, 13, 1, 3, 7, 13, 15, 5, 9, 11, 15, 5, 11, 13, 3, 7, 9, 15, 3, 9, 1. We multiply all of these numbers modulo 16, taking advantage of the fact that $3\cdot 5 \equiv -1 (\text{mod }16)$, $7\cdot9\equiv -1 (\text{mod }16)$, $11\cdot 13\equiv -1 (\text{mod }16)$, and $15\equiv -1(\text{mod }16)$. We find that our answer is $\boxed{6}$.
overlap: 
between 1 and 100 are 2, 3, 5, 7, 11, 13, 17, 19, 23, 29, 31, 37, 41, 43, 47, 53, 59, 61, 67, 71, 73, 79, 83, 89, and 97.
>>>>>>>>

output:  458
The sum of the first $n$ odd integers is $1 + 3 + \dots + (2n - 1)$. The sum of an arithmetic series is equal to the average of the first and last term, multiplied by the number of terms, so this sum is $[1 + (2n - 1)]/2 \cdot n = n^2$. Then the sum of the odd integers between 0 and 100 is $50^2$, and the sum of the odd integers between 0 and 200 is $100^2$. Therefore, the ratio of the sum of the odd integers between 0 and 100 to the sum of the odd integers between 100 and 200 is $\frac{50^2}{100^2-50^2}=\frac{1}{4-1}=\boxed{\frac{1}{3}}$.
overlap: 
+ \dots + (2n - 1)$. The sum of an arithmetic series is equal to the average of the first and last term, multiplied by the number of terms, so
>>>>>>>>

output:  3562
Let's find the cycle of units digits of $7^n$, starting with $n=1$ : $7, 9, 3, 1, 7, 9, 3, 1,\ldots$ . The cycle of units digits of $7^{n}$ is 4 digits long: 7, 9, 3, 1. Thus, to find the units digit of $7^n$ for any positive $n$, we must find the remainder, $R$, when $n$ is divided by 4 ($R=1$ corresponds to the units digit 7, $R=2$ corresponds to the units digit 9, etc.) Since $53\div4=13R1$, the units digit of $7^{53}$ is $\boxed{7}$.
overlap: 
$7, 9, 3, 1, 7, 9, 3, 1,\ldots$ . The cycle of units digits of $7^{n}$ is 4 digits long: 7, 9, 3, 1. Thus, to find the units digit of $7^n$ for any positive $n$, we must find the remainder, $R$, when $n$ is divided by 4 ($R=1$ corresponds to the units digit 7, $R=2$ corresponds to the units digit 9, etc.) Since
>>>>>>>>

output:  2349
Note that \[ab + bc + cd \le ab + bc + cd + da = (a + c)(b + d).\]By AM-GM, \[(a + c)(b + d) \le \left( \frac{(a + c) + (b + d)}{2} \right)^2 = \frac{1}{4}.\]Equality occurs when $a = 0,$ $b = \frac{1}{2},$ $c = \frac{1}{2},$ and $d = 0,$ so the maximum value of $ab + bc + cd$ is $\boxed{\frac{1}{4}}.$
overlap: 
that \[ab + bc + cd \le ab + bc + cd + da = (a + c)(b + d).\]By AM-GM, \[(a + c)(b + d) \le \left( \frac{(a + c) + (b + d)}{2} \right)^2 =
>>>>>>>>

output:  333
Let $d$ be the common difference. Then the last term is $7 + (15-1)d = 7+14d$. The sum of an arithmetic series is equal to the average of the first and last term, multiplied by the number of terms, so the sum of the series is \[\frac{7 + (7 + 14d)}{2} \cdot 15 = 15(7d + 7) = 105d + 105.\]We are told that this sum equals $-210$, so we have $105+105d = -210$, from which we find $d=\boxed{-3}$. Note: $\boxed{3}$ is also accepted as an answer.
overlap: 
The sum of an arithmetic series is equal to the average of the first and last term, multiplied by the number of terms, so the sum of the series is
>>>>>>>>

output:  3695
The measure of each interior angle in a regular $n$-gon is $180(n-2)/n$ degrees. Therefore, the measure of angle $\angle BAD$ is $180(6-2)/6=120$ degrees and the measure of angle $CAD$ is 108 degrees. Their difference, $\angle BAC$, measures $120-108=\boxed{12\text{ degrees}}$.
overlap: 
The measure of each interior angle in a regular $n$-gon is $180(n-2)/n$ degrees. Therefore, the measure of angle $\angle BAD$ is $180(6-2)/6=120$ degrees and the measure of angle $CAD$ is
>>>>>>>>

output:  79
The radius of the circular path of the horse closer to the center is $\frac{1}{4}$ of the radius of the path of the horse farther from the center. Since circumference is directly proportional to radius, the length of shorter path is $\frac{1}{4}$ of the length of the longer path. Therefore, 4 times as many revolutions must be made to go the same distance, which is $27\times4=\boxed{108}$ revolutions.
overlap: 
radius of the circular path of the horse closer to the center is $\frac{1}{4}$ of the radius of the path of the horse farther from the center. Since circumference is directly proportional to radius, the length of
>>>>>>>>

output:  593
Moving terms to the LHS, we have $x^2-6x+y^2+8y=24$. Completing the square on the quadratic in $x$, we add $(6/2)^2=9$ to both sides. Completing the square on the quadratic in $y$, we add $(8/2)^2=16$ to both sides. We are left with the equation $x^2-6x+9+y^2+8y+16=49 \Rightarrow (x-3)^2+(y+4)^2=49$. Thus, our circle has center $(3,-4)$. The distance between this center and the point $(-3,-12)$ is $\sqrt{(-3-3)^2+(-12-(-4))^2}=\boxed{10}$.
overlap: 
Completing the square on the quadratic in $x$, we add $(6/2)^2=9$ to both sides. Completing the square on the quadratic in $y$, we add $(8/2)^2=16$ to both sides. We are left with the equation
>>>>>>>>

output:  4816
By the product-to-sum identities, we have that $2\cos a \sin b = \sin (a+b) - \sin (a-b)$. Therefore, this reduces to a telescoping series: \begin{align*} \sum_{k=1}^{n} 2\cos(k^2a)\sin(ka) &= \sum_{k=1}^{n} [\sin(k(k+1)a) - \sin((k-1)ka)]\\ &= -\sin(0) + \sin(2a)- \sin(2a) + \sin(6a) - \cdots - \sin((n-1)na) + \sin(n(n+1)a)\\ &= -\sin(0) + \sin(n(n+1)a)\\ &= \sin(n(n+1)a). \end{align*}Thus, we need $\sin \left(\frac{n(n+1)\pi}{2008}\right)$ to be an integer; this integer can be only $\{-1,0,1\}$, which occurs when $2 \cdot \frac{n(n+1)}{2008}$ is an integer. Thus $1004 = 2^2 \cdot 251$ divides $n(n+1)$. Since 251 is prime, 251 must divide $n$ or $n + 1.$ The smallest such $n$ is 250, but 1004 does not divide $250 \cdot 251.$ The next smallest such $n$ is 251, and 1004 divides $251 \cdot 252.$ Therefore, the smallest such integer $n$ is $\boxed{251}.$
overlap: 
we have that $2\cos a \sin b = \sin (a+b) - \sin (a-b)$. Therefore, this reduces to a telescoping series: \begin{align*} \sum_{k=1}^{n} 2\cos(k^2a)\sin(ka) &= \sum_{k=1}^{n} [\sin(k(k+1)a) - \sin((k-1)ka)]\\ &= -\sin(0) + \sin(2a)- \sin(2a) + \sin(6a) - \cdots - \sin((n-1)na) + \sin(n(n+1)a)\\ &= -\sin(0) +
>>>>>>>>

output:  2959
Let $x = \frac{a}{b},$ $y = \frac{b}{c},$ and $z = \frac{c}{a}.$ Then $x + y + z = 7$ and $\frac{1}{x} + \frac{1}{y} + \frac{1}{z} = 9.$ Also, \[xyz = \frac{a}{b} \cdot \frac{b}{c} \cdot \frac{c}{a} = 1,\]so $xy + xz + yz = 9.$ We want to compute $x^3 + y^3 + z^3.$ Recall the factorization \[x^3 + y^3 + z^3 - 3xyz = (x + y + z)(x^2 + y^2 + z^2 - xy - xz - yz).\]Squaring the equation $x + y + z = 7,$ we get \[x^2 + y^2 + z^2 + 2(xy + xz + yz) = 49.\]Then \[x^2 + y^2 + z^2 - xy - xz - yz = 49 - 3(xy + xz + yz) = 49 - 3 \cdot 9 = 22.\]Hence, \[x^3 + y^3 + z^3 = 7 \cdot 22 + 3 = \boxed{157}.\]
overlap: 
the factorization \[x^3 + y^3 + z^3 - 3xyz = (x + y + z)(x^2 + y^2 + z^2 - xy - xz - yz).\]Squaring the equation $x + y + z =
>>>>>>>>

output:  1237
We consider the subset $\{ 2, 3, 5, 7, 11 \}$ which consists only of the prime integers in the original set. Any subset consisting entirely of prime numbers must be a subset of this particular subset. And, there are $2^5 - 1 = \boxed{31}$ non-empty subsets of this 5-element set, which we can easily see by making the choice of including or not including each element.
overlap: 
numbers must be a subset of this particular subset. And, there are $2^5 - 1 = \boxed{31}$ non-empty subsets of this 5-element set, which we can easily see by making the choice of including or not including each element.
>>>>>>>>

output:  503
The function is defined when the value inside the square root is positive, i.e. we must have $x^2-5x+6>0$. Factoring, we get $(x-3)(x-2)>0$. So either both factors in the left hand side are negative or they are both positive. They are both negative when $x<2$. They are both positive when $x>3$. So the domain of $f(x)$ is $x<2 \text{ or } x>3$, or $x \in \boxed{(-\infty, 2) \cup (3, \infty)}$ in interval notation.
overlap: 
So either both factors in the left hand side are negative or they are both positive. They are both negative when $x<2$. They are both positive when $x>3$. So the domain of
>>>>>>>>

output:  4954
Let $\mathbf{v} = \begin{pmatrix} 3 \\ 6 \\ 15 \end{pmatrix}$ and $\mathbf{w} = \begin{pmatrix} 2 \\ 1 \\ -2 \end{pmatrix}.$ [asy] import three; size(180); currentprojection = perspective(6,3,2); triple I = (1,0,0), J = (0,1,0), K = (0,0,1), O = (0,0,0); triple V = (3,2,2), W = (4,1,3), P = dot(V,W)/abs(W)^2*W, R = 2*P - V; draw(V--R,dashed); draw(0.85*P--(0.85*P + 0.15*(V - P))--(P + 0.15*(V - P))); draw(O--V,Arrow3(6)); draw(P--W,Arrow3(6)); draw(O--P,Arrow3(6)); draw(O--R,Arrow3(6)); draw(O--3*I, Arrow3(6)); draw(O--3*J, Arrow3(6)); draw(O--3*K, Arrow3(6)); label("$x$", 3.2*I); label("$y$", 3.2*J); label("$z$", 3.2*K); label("$\mathbf{v}$", V, NE); label("$\mathbf{w}$", W, N); label("$\mathbf{p}$", P, SW); label("$\mathbf{r}$", R, SW); [/asy] Let $\mathbf{p}$ be the projection of $\mathbf{v}$ onto $\mathbf{w},$ so \[\mathbf{p} = \frac{\mathbf{v} \cdot \mathbf{w}}{\mathbf{w} \cdot \mathbf{w}} \mathbf{w} = \frac{\begin{pmatrix} 3 \\ 6 \\ 15 \end{pmatrix} \cdot \begin{pmatrix} 2 \\ 1 \\ -2 \end{pmatrix}}{\begin{pmatrix} 2 \\ 1 \\ -2 \end{pmatrix} \cdot \begin{pmatrix} 2 \\ 1 \\ -2 \end{pmatrix}} \begin{pmatrix} 2 \\ 1 \\ -2 \end{pmatrix} = \frac{-18}{9} \begin{pmatrix} 2 \\ 1 \\ -2 \end{pmatrix} = \begin{pmatrix} -4 \\ -2 \\ 4 \end{pmatrix}.\]Let $\mathbf{r}$ be the reflection of $\mathbf{v}$ across line $L.$ Then $\mathbf{p}$ is the midpoint of $\mathbf{v}$ and $\mathbf{r},$ so \[\mathbf{p} = \frac{\mathbf{v} + \mathbf{r}}{2}.\]Then \[\mathbf{r} = 2 \mathbf{p} - \mathbf{v} = 2 \begin{pmatrix} -4 \\ -2 \\ 4 \end{pmatrix} - \begin{pmatrix} 3 \\ 6 \\ 15 \end{pmatrix} = \begin{pmatrix} -11 \\ -10 \\ -7 \end{pmatrix}.\]Hence, the resulting point is $\boxed{(-11,-10,-7)}.$
overlap: 
\end{pmatrix} \cdot \begin{pmatrix} 2 \\ 1 \\ -2 \end{pmatrix}}{\begin{pmatrix} 2 \\ 1 \\ -2 \end{pmatrix} \cdot \begin{pmatrix} 2 \\ 1 \\ -2 \end{pmatrix}} \begin{pmatrix} 2 \\ 1 \\ -2 \end{pmatrix} =
>>>>>>>>

output:  701
We see that $x^2 + 4x + 4 = (x + 2)^2$. If $x$ must be positive, we can see that this expression can take on the value of any perfect square that is greater than or equal to $(1+2)^2=9$. The possible values between 10 and 50 are thus 16, 25, 36, and 49, achieved when $x=2,3,4,5$ respectively. So, there are $\boxed{4}$ positive integers $x$ for which $x^2+4x+4$ is between 10 and 50.
overlap: 
see that $x^2 + 4x + 4 = (x + 2)^2$. If $x$ must be positive, we can see that this expression can take on the value of any perfect square that is greater than or equal to
>>>>>>>>

\end{lstlisting}



==> tables/data_construction.tex <==
\begin{table}[t]
\caption{The composition of KPMath-Plus.}
\label{tab:data_construction}
% \vskip 0.05in
\begin{center}
% \resizebox{\columnwidth}{!}{%
\begin{small}
\begin{tabular}{lrrr}
\toprule
Data & \#~Samples & \#~Epochs & Proportion \\
\midrule
MMIQC & 2.29M & 1 & 59.3\%\\
MathInstruct-CoT & 188K & 3 & 14.6\%\\
KPMath & 1.01M & 1 & 26.1\%\\
\midrule
KPMath-Plus & 3.86M & - & 100\% \\
\bottomrule
\end{tabular}
\end{small}
% }
\end{center}
% \vskip -0.1in
\end{table}


==> tables/full_results.tex <==

\begin{table}[t]
\caption{Results on 9 mathematical reasoning tasks. MAWPS results are averaged over four tasks: Singleeq, Singleop, Addsub, and MultArith. Vanilla models are tested with CoT. The best results in each section are in \colorbox{lightblue}{blue}, the second-best results are underlined, while the results of our best model are bolded. $^*$ ZS: Zero-shot inference without demonstrations.
}
\label{tab:main}
\centering
\setlength{\tabcolsep}{4pt}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lrcc|cccccc|c}
\toprule
\textbf{Model} & \textbf{Size} & \textbf{Tools} & \textbf{ZS$^*$} & \textbf{GSM8k} & \textbf{MATH} & \textbf{SVAMP} & \textbf{TabMWP} & \textbf{ASDiv} & \multicolumn{1}{c|}{\textbf{MAWPS}} & \multirow{2}{*}{\textbf{AVG}} \\
\cmidrule{1-10}
\multicolumn{4}{l|}{\textbf{Used as Seed Data?}} & \cmark & \cmark & \xmark & \xmark & \xmark & \xmark & \\
\midrule
\multicolumn{11}{c}{Proprietary Models} \\
\midrule
GPT-4 & - & \xmark & \xmark &  92.0 & 42.5 & 93.1 & 67.1 & 91.3 & 97.6 & 80.6 \\
GPT-4 (PAL) \code & - & \cmark & \xmark & 94.2 & 51.8  & 94.8 & 95.9 & 92.6 & 97.7 & 87.8 \\
\midrule
ChatGPT & - & \xmark & \xmark & 80.8 & 35.5  & {83.0} & {69.1} & {87.3} & {94.6} & 75.1 \\
ChatGPT (PAL) \code & - & \cmark & \xmark & {78.6} & {38.7} & 77.8 & {79.9} & {81.0} & 89.4 & 74.2 \\
Claude-2 & - & \xmark & \xmark & {85.2} & 32.5  & - & - & - & - & - \\
PaLM-2 & 540B & \xmark & \xmark & 80.7 & {34.3} & - & - & - & - & - \\
 \midrule
\multicolumn{11}{c}{Open-Source Models} \\
 \midrule
LLaMA-2 & 7B & \xmark & \xmark & 13.3 & 4.1  & 38.0 & 31.1 & 50.7 & 60.9 & 33.0 \\
LLaMA-2 SFT & 7B & \xmark & \cmark & 41.3 & 7.2  & 31.9 & 27.8 & 47.4 & 60.0 & 35.9 \\
Mistral & 7B & \xmark & \xmark & 42.9 & 12.9  & 65.1 & 55.6 & 68.4 & 86.8 & 55.3 \\
% LLaMA-2 RFT & 7B & \xmark & \cmark & 51.2 & - & - & - & - & - & -\\
Platypus-2 & 7B & \xmark & \xmark & 14.4 & 5.4 & 36.7 & 26.5 & 47.9 & 58.4 & 31.6 \\
WizardMath & 7B & \xmark & \cmark & 54.9 & 10.7 & 57.3 & 38.1 & 59.1 & 73.7 & 49.0 \\
CodeLLaMA (PAL) \code & 7B & \cmark & \xmark & 34.0 & 16.6 & 59.0 & {47.3} & 61.4 & 79.6 & 49.7 \\
% Toolformer \calc & 7B & \cmark & \cmark & - & - & 29.4 & - & 40.4 & 44.0 & - \\
MetaMath-7B  & 7B &  \\
Mistral-7B-MetaMathQA  & 7B &  \\
ToRA & 7B & \cmark & \cmark & 68.8 & 40.1 & 68.2 & 42.4 & 73.9 & 88.8 & 63.7 \\
ToRA-Code & 7B & \cmark & \cmark & 72.6 & 44.6 & 70.4 & 51.6 & 78.7 & 91.3 & 68.2 \\
KPMath-Plus-Mistral & 7B & \xmark & \cmark & \blue{\textbf{82.1}} & \blue{\textbf{46.8}} & \blue{\textbf{76.4}} & \blue{\textbf{66.4}} & \blue{\textbf{86.7}} & \blue{\textbf{94.2}} & \blue{\textbf{75.4~\small{(+20.1)}}} \\
% KPMath-Plus-Mistral-7B & 7B & \cmark & \cmark & \blue{\textbf{81.7}} & \blue{\textbf{46.1}} & \blue{\textbf{75.9}} & \blue{\textbf{67.7}} & \blue{\textbf{86.1}} & \blue{\textbf{93.8}} & \blue{\textbf{75.2~\small{(+)}}} \\
% KPMath-Plus-Mistral-7B-2 & 7B & \cmark & \cmark & \blue{\textbf{79.9}} & \blue{\textbf{46.6}} & \blue{\textbf{78.4}} & \blue{\textbf{66.6}} & \blue{\textbf{87.1}} & \blue{\textbf{93.6}} & \blue{\textbf{75.36~\small{(+)}}} \\
\midrule

LLaMA-2 & 13B & \xmark & \xmark & 24.3 & 6.3 & 43.1 & 39.5 & 56.3 & 70.4 & 36.2 \\
LLaMA-2 SFT & 13B & \xmark & \cmark &  51.1 & 9.2 & 46.3 & 35.8 & 58.6 & 75.0 & 42.6 \\
% LLaMA-2 RFT & 13B & \xmark & \cmark & 55.3 & - & - & - & - & - & -\\
Platypus-2 & 13B & \xmark & \xmark & 23.7 & 7.1 & 50.7 & 45.3 & 55.1 & 69.6 & 38.0 \\
WizardMath & 13B & \xmark & \cmark & 63.9 & 14.0 & 64.3 & 46.7 & 65.8 & 79.7 & 51.8 \\
CodeLLaMA (PAL)  & 13B & \cmark & \xmark & 39.9 & 19.9 & 62.4 & {59.5} & 65.3 & 86.0 & 53.1 \\

ToRA & 13B & \cmark & \cmark & {72.7} & {43.0} & {72.9} & 47.2 & {77.2} & {91.3} & {65.9} \\
ToRA-Code & 13B & \cmark & \cmark & 
75.8 & 48.1 & 60.5 & 65.4 & 81.4 & 92.5 & 71.3 \\
\midrule
% LLaMA-1 RFT & 34B & \xmark & \cmark & 57.9 & - & - & - & - & - & -\\
CodeLLaMA (PAL) \code & 34B & \cmark & \xmark & 53.3 & 23.9 & 71.0 & 63.1 & 72.4 & 91.5 & 60.7\\
Llemma-34B-MetaMathQA  & 34B &  \\
Llemma-34B-MMIQC  & 34B &  \\
ToRA-Code & 34B & \cmark & \cmark & 80.7 & 50.8 & 80.5 & 70.5 & 84.2 & 93.3 & 74.8 \\
\midrule

LLaMA-2 & 70B & \xmark & \xmark & 57.8 & 14.4& 73.6 & 57.5 & 76.0 & 92.4 & 58.2 \\
LLaMA-2 SFT & 70B & \xmark & \cmark & 69.3 & 14.9 & 64.0 & 53.0 & 71.3 & 84.8 & 56.6 \\
% LLaMA-2 RFT & 70B & \xmark & \cmark & 64.8 & - & - & - & - & - & -\\
Platypus-2 & 70B & \xmark & \xmark & 45.9 & 15.0 & 74.3 & 47.3 & 72.7 & 91.1 & 53.0 \\
WizardMath & 70B & \xmark & \cmark & {81.6} & {22.7} & {80.0} & 49.8 & {76.2} & 86.2 & {63.8} \\
LLaMA-2 (PAL) \code & 70B & \cmark & \xmark & 55.2 & 18.3 & 74.6 & {59.5} & 71.9 & {92.8} & 60.3 \\

ToRA & 70B & \cmark & \cmark & 84.3 & 49.7 & 82.7 & 74.0 & 86.8 & 93.8 & 76.9 \\
\bottomrule
\end{tabular}
}%
\end{table}




==> tables/result_1.tex <==
\begin{table*}[t]
\caption{PASS@1 Accuracy (\%) on MATH dataset. The models marked with an asterisk (*) are evaluated by us. Our fine-tuned 7B model surpasses all non-code 7B models and even outperforms some 34B models.}
\label{tab:math-acc}
% \vskip 0.15in
\begin{center}
\begin{small}
% \begin{sc}
\resizebox{1.0\textwidth}{!}{%
\begin{tabular}{lccccc}
\toprule
Model      & FT-Dataset & Code & Zero-shot  &  MATH & GSM8K \\
\midrule
Proprietary Models \\
\midrule
\quad Claude-2~\citep{anthropic2023claude} & - & \xmark & \xmark & 32.5 &  \\
\quad PaLM-2~\citep{anil2023palm} & - & \xmark & \xmark & 34.3 &  \\
\quad ChatGPT (GPT-3.5) & - & \xmark & \xmark & 35.5 &  \\
\quad GPT-4 {\tiny(2023-0314)}~\citep{openai2023gpt4} & - & \xmark & \cmark & 42.5  &  \\
\quad Gemini-Ultra~\citep{team2023gemini} & - & \xmark & \xmark & 53.2 &  \\
\midrule
Open-Source Models \\
% $\sim$7B models \\
\midrule
\quad Llama-2-7B~\citep{Touvron2023Llama2O} & - & \xmark & \xmark & 4.1  &  \\
\quad WizardMath-7B~\citep{luo2023wizardmath} & WizardMath & \xmark & \cmark & 10.7  &  \\
% \quad Qwen-7B~\citep{bai2023qwen} & - & \xmark & \xmark & 11.6  &  \\
\quad Llemma-7B~\citep{azerbayev2023llemma} & Proof-Pile-2 & \xmark & \cmark & 18.0  &  \\
\quad MetaMath-7B~\citep{yu2023metamath} & MetaMathQA & \xmark & \cmark &  19.8  &  \\
% 8-shot
\quad Mistral-7B~\citep{jiang2023mistral}  & - & \xmark  & \xmark & 10.5*   &  \\
\quad Mistral-7B-MetaMathQA~\citep{yu2023metamath}  & MetaMathQA & \xmark  & \cmark & 28.2   &  \\
\quad Mistral-7B-MMIQC~\citep{liu2024augmenting}    & MMIQC & \xmark & \cmark    &  36.0  &  \\
\quad MAmmoTH-Coder-7B~\citep{yue2023mammoth} & MathInstruct & \cmark & \cmark & 33.4  &  \\
\quad MathGenieLM \\
% \quad Xwin-Math \\
% \quad MathScale \\
% \quad ToRA-Code-7B~\citep{gou2023tora}  & ToRA-Corpus & \cmark & \cmark &  44.6  &  \\
% \midrule
% $\sim$34B models \\
% \midrule
\quad CodeLlamma-34B~\citep{codellama} & - & \cmark  & \xmark & 25.0  &  \\
\quad Llemma-34B-MetaMathQA~\citep{yu2023metamath}  & MetaMathQA & \xmark  & \cmark & 34.8  &  \\
\quad Llemma-34B-MMIQC~\citep{liu2024augmenting}  & MMIQC & \xmark & \cmark & 38.6  &  \\
% \quad Llemma-34B-MetaMathQA & MetaMathQA & Math-Shepherd  & maj+verify1@256 &  47.3 \\
% \quad ToRA-Code-34B~\citep{gou2023tora}  & ToRA-Corpus & \cmark & \cmark &  50.8 \\
% \midrule
% $\sim$70B models \\
% \midrule
% \quad Llama-2-70B~\citep{Touvron2023Llama2O} & - & \xmark & \xmark & 13.5 \\
% \quad WizardMath-70B~\citep{luo2023wizardmath} & WizardMath & \xmark & \cmark & 22.7 \\
% \quad DeepSeek-67B~\citep{bi2024deepseek} & - & \xmark & \xmark & 18.7 \\
% \quad Deepseek-67B-MetaMathQA~\citep{yu2023metamath}   & MetaMathQA &  \xmark  & \cmark &  36.8 \\
% \quad Deepseek-67B-MMIQC~\citep{liu2024augmenting}   & MMIQC &  \xmark  & \cmark &  41.0 \\
% \quad Deepseek-67B-MetaMathQA  & MetaMathQA &  \xmark  & maj1@256 &  45.4 \\
% \quad Deepseek-67B-MetaMathQA  & MetaMathQA &  Math-Shepherd  & maj+verify1@256 &  48.1 \\
% \quad Qwen-72B~\citep{bai2023qwen}  & - &  \xmark  & \cmark &  35.2 \\
% \quad Qwen-72B-MetaMathQA~\citep{yu2023metamath}  & MetaMathQA &  \xmark  & \cmark &  41.7 \\
% \quad Qwen-72B-MMIQC~\citep{liu2024augmenting}   & MMIQC &  \xmark  & \cmark &  45.0 \\
\midrule
\quad \textbf{Mistral-7B-KPMath-Plus} & \textbf{KPMath-Plus} &  \xmark  & \cmark &  \textbf{39.3*} \\
\bottomrule
\end{tabular}
}
% \end{sc}
\end{small}
\end{center}
% \vskip -0.1in
\end{table*}
